Hecke modifications of Higgs bundles and the extended Bogomolny equation

We establish a Kobayashi-Hitchin correspondence between solutions of the extended Bogomolny equation with a Dirac type singularity and Hecke modifications of Higgs bundles. This correspondence was conjectured by Witten and plays an important role in the physical description of the the geometric Langlands program in terms of S-duality for N=4 super Yang-Mills theory in four dimensions.

==> GCHeckeModifications.tex <==
\section{Hecke modifications of $G^\C$ Higgs bundles}
\label{Sec_HeckeModificationsOfGCHiggsBundles}

This appendix discusses the extension of \autoref{Thm_EBE=Hecke} to Hecke modifications of $G^\C$ Higgs bundles.
Throughout, let $G$ be a compact, connected Lie group, denote by $G^\C$ its complexification, and let $\Sigma$ be a Riemann surface.

\begin{definition}
  \label{Def_GCHiggsBundle}
  A \defined{$G^\C$ Higgs bundle} over $\Sigma$ is a holomorphic $G^\C$--principal bundle $\pi\co \sP \to \Sigma$ together with a holomorphic $1$--form $\varphi \in H^0(\Sigma,K_\Sigma\otimes\Ad(\sP))$.
\end{definition}

Let $P$ be a principal $G$--bundle over $\Sigma$ and denote by $P^\C \coloneq P\times_G G^\C$ the induced principal $G^c$--bundle.
Denote by $\pi\co P^\C \to \Sigma$ the projection map
A connection $A \in \sA(P)$ on $P$ induces a decomposition $TP^\C \iso \pi^*T\Sigma \oplus P^\C\times \fg^\C$.
Define an almost complex structure $I_A$ on $P^\C$ by
\begin{equation}
  \label{Eq_IA}
  I_A \coloneq \pi^*I_\Sigma \oplus i.
\end{equation}
Since $F_A^{0,2} = 0$, the Nijenhuis tensor of $I_A$ vanishes.
Therefore, $I_A$ is integrable and makes $P^\C$ into a holomorphic principal bundle which we denote by $\sP_A$.
In fact, as was observed by \citet{Singer1959}, this construction induces a one-to-one correspondence between connections on $A$ and holomorphic structures on $P^\C$ making it into a holomorphic principal bundle.
If $\phi \in \Omega^1(\Sigma,\Ad(P))$, then
\begin{equation}
  \varphi \coloneq \frac12(\phi - iI_\Sigma\phi)
\end{equation}
is a section of $K_\Sigma\otimes\Ad(\sP_A)$.
It follows from the Kähler identities that $\varphi$ is holomorphic if and only if $\rd_A \phi = 0$ and $\rd_A^* \phi = 0$.

There is a notion of $\mu$--polystability for $G^\C$ Higgs bundles and $(\sP,\varphi)$ is
XXX Hitchin equation
admits a Hermitian metric $H$ such that $(A,\phi)$ satisfies \defined{Hitchin's equation}
\begin{equation}
  \label{Eq_Hitchin}
  F_A^\circ - \frac12[\phi\wedge \phi] = 0, \quad
  \rd_A \phi = 0, \qandq
  \rd_A^* \phi = 0
\end{equation}
if and only if it is $\mu$--polystable.
XXX


\begin{definition}
  \label{Def_HeckeModification}
  Let $z \in \Sigma$ and $w\co \U(1) \to G$ be a dominant coweight.
  A \defined{Hecke modification} of a $G^\C$ Higgs bundle $(\sP,\varphi)$ at $z$ of type $w$ is a $G^\C$ Higgs bundle $(\sQ,\chi)$ together with an isomorphism
  \begin{equation}
    \eta\co (\sP,\phi)|_{\Sigma\setminus\set{z}} \iso (\sQ,\chi)|_{\Sigma\setminus\set{z}} 
  \end{equation}
  of $G^\C$ Higgs bundles which, in suitable trivializations near $z$, is given by the complexification of $w$.

  An \defined{isomorphism} between two Hecke modification $(\sQ_1,\chi_1;\eta_1)$ and $(\sQ_2,\chi_2;\eta_2)$ of $(\sP,\varphi)$ is isomorphism
  \begin{equation}
    \xi\co (\sQ_1,\chi_1) \to (\sQ_2,\chi_2)
  \end{equation}
  such that
  \begin{equation}
    \eta_1 = \eta_2\xi.
  \end{equation}
  We denote by
  \begin{equation}
    \sM^\Hecke(\sP,\varphi;z,w)
  \end{equation}
  the set of all isomorphism classes of Hecke modifications of $(\sP,\varphi)$ at $z$ of type $w$.  
\end{definition}

Throughout, let $M$ be an oriented Riemannian $3$--manifold.

\begin{definition}
  \label{Def_EBE}
  Let $P$ be a principal $G$--bundle over $M$.
  The \defined{extended Bogomolny equation} is the following partial differential equation for
  a connection $A \in \sA(P)$,
  a $1$--form $\phi \in \Omega^1(M,\Ad(P))$,
  and section $\xi \in \Omega^0(M,\Ad(P))$:
  \begin{equation}
    \label{Eq_EBE}
    \begin{split}
      F_A - \frac12[\phi\wedge\phi] &= *\rd_A\xi, \\
      \rd_A\phi - *[\xi,\phi] &= 0, \qand \\
      \rd_A^*\phi &= 0.
    \end{split}
  \end{equation}
\end{definition}

In this article, we are exclusively concerned with singular solutions of \autoref{Eq_EBE}.
The following example is archetypical.

\begin{example}
  \label{Ex_DiracMonopole}
  Denote by $Q \to S^2$ the principal $\U(1)$--bundle with $c_1(Q) = 1$.
  This can be realized, e.g., as the unit sphere bundle of $\sO_{\CP^1}(1)$.
  $Q$ admits a connection $B$ with curvature
  \begin{equation}
    F_B = -\frac{i}{2}\vol_{S^2}.
  \end{equation}
  Denote by $\pi\co \R^3\setminus\set{0} \to S^2$ the projection map.
  Denote by $r\co \R^3 \to [0,\infty)$ the distance to the origin.
  Set
  \begin{equation}
    P \coloneq \pi^*Q, \quad
    A \coloneq \pi^*B, \qandq
    \xi \coloneq \frac{i}{2r}
  \end{equation}
  The pair $(A,\xi)$ satisfies the Bogomolny equation
  \begin{equation}
    F_A = *\rd_A \xi
  \end{equation}
  and thus \autoref{Eq_EBE} with $\phi = 0$.
\end{example}

\begin{definition}
  Given a coweight $w\co \U(1) \to G$,
  set
  \begin{equation}
    P_w \coloneq P\times_{\U(1)} G
  \end{equation}
  and denote by $A_w$ the connection on $P_w$ induced by $A$ and by $\xi_w$ the section of $\Ad(P)$ induced by $\xi$.
  We call the pair
  \begin{equation}
    (A_w,\xi_w)
  \end{equation}
  the \defined{Dirac monopole} of coweight $w$.
\end{definition}

% XXX I'm not happy with the language here yet.  The bundle does know its coweight.

\begin{definition}
  \label{Def_Framing}
  Let $p \in M$,
  let $P$ be a principal $G$--bundle over $M\setminus \set{p}$, and
  let $w \co \U(1) \to G$ be a coweight.
  A \defined{framing} of $P$ at $p$ of coweight $w$ is an isomorphism
  \begin{equation*}
    \Psi\co (\exp_p^*P)|_{B_r(0)} \to P_w|_{B_r(0)}.
  \end{equation*}
  Here $r > 0$ is one half of the injectivity radius of $M$ at $p$.
  The pair $(P,\Psi)$ is called a \defined{$(p,w)$--framed} principal $G$--bundle.
\end{definition}

\begin{definition}
  \label{Def_DiracTypeSingularity}
  Let $(P,\Psi)$ be a $(p,w)$--framed principal $G$--bundle.
  A solution $(A,\phi,\xi)$ of \autoref{Eq_EBE} on $P$ is said to have a \defined{Dirac type singularity} with coweight $w$ at $p$ if there exists an $\alpha > 0$ such that
  \begin{equation}
    \label{Eq_DiracTypeSingularity}
    \Psi_*A = A_w + O(r^{-1+\alpha}), \quad
    \Psi_*\phi = O(1), \qandq
    \Psi_*\xi = \xi_w + O(r^{-1+\alpha}).
  \end{equation}
\end{definition}

\begin{definition}
  Let $(P,\Psi)$ be a $(p,w)$--framed principal $G$--bundle.
  A  gauge transformation $u \in \sG(P)$ is called \defined{singularity preserving} if there exists a $u_p \in \sG(P_w)$ such that
  \begin{equation*}
    (u_p)_*A_w = A_w \qandq
    (u_p)_*\xi_w = \xi_w
  \end{equation*}
  and an $\alpha > 0$ such that
  \begin{equation}
    d(\Psi_*u,u_p) = O(r^\alpha) \qandq
    \nabla_{A_w}(\Psi_*u) = O(r^{-1+\alpha}).
  \end{equation}
\end{definition}

\begin{remark}
  If $(A,\phi,\xi)$ has a Dirac type singularity and $u$ is singularity preserving,
  then $u_*(A,\phi,\xi)$ also has a Dirac type singularity.
\end{remark}


Let $\Sigma$ be a closed Riemann surface,
let $P_0$ be a principal $G$--bundle over $\Sigma$, and
let $(A_0,\phi_0)$ be a solution of Hitchin's equation on $P_0$.
Let $p = (y_0,z_0) \in (0,1)\times \Sigma$ and let $w \co \U(1) \to G$ be a coweight.
There exists a $(p,w)$--framed principal $G$--bundle $(P,\Psi)$ over $[0,1]\times\Sigma\setminus\set{p}$ which agrees with $P_0$ over $\set{0}\times \Sigma$.
Furthermore, any two choices of $(P,\Psi)$ are isomorphic.
Throughout, we fix such a such a choice.

\begin{definition}
  \label{Def_MEBE}
  Denote by $\sC^\EBE(A_0,\phi_0;p,w)$ the set of triples $A \in \sA(P)$, $\phi \in \Omega^1([0,1]\times\Sigma\setminus\set{p},\Ad(P))$, and $\xi \in \Omega^0([0,1]\times\Sigma\setminus\set{p},\Ad(P))$ satisfying the extended Bogomolny equation \autoref{Eq_EBE} as well as
  \begin{equation}
    \label{Eq_IDelYPhi=0}
    i(\del_y)\phi = 0;
  \end{equation}
  and the boundary conditions
  \begin{equation}
    \label{Eq_BoundaryConditions}
    A|_{\set{0}\times\Sigma} = A_0, \quad
    \phi|_{\set{0}\times\Sigma} = \phi_0, \qandq
    \xi|_{\set{1}\times\Sigma} = 0.
  \end{equation}
  Denote by $\sG$ the group of singularity preserving unitary gauge transformations of $P$ which restrict to the identity on $\set{0}\times \Sigma$.
  We set
  \begin{equation}
    \sM^\EBE(A_0,\phi_0;(y,z),w)
    \coloneq
    \sC^\EBE(A_0,\phi_0;(y,z),w)/\sG.
  \end{equation}
\end{definition}

\begin{remark}
  It is an interesting question to ask whether the condition \autoref{Eq_IDelYPhi=0} really does need to be imposed.
  In a variant of this setup on $S^1\times \Sigma$, the condition is automatically satisfied.
\end{remark}

A connection $A \in \sA(P)$ induces an endomorphism $I = I_A \in \Gamma(\End(TP^\C))$ which induces a complex structure on the restriction over $\set{y}\times \Sigma$ which makes $P^\C|_{\set{y}\times\Sigma}$ into a holomorphic principal $G^\C$--bundle.
The connection also induces a horizontal vector field $\tilde\del_y \in \Vect(P^\C)$ which lifts $\del_y$.
Thinking of $\xi$ as a vertical vector field on $TP^\C$ we set
\begin{equation*}
  \fd_y \coloneq \tilde\del_y - i\xi \in \Vect(P^\C).
\end{equation*}
If $\phi$ satisfies \autoref{Eq_IDelYPhi=0},
then
\begin{equation*}
  \phi = \varphi - \varphi^*
  \qwithq
  \varphi \coloneq \frac12(\phi - iI_\Sigma\phi) \qandq
  \varphi^* \coloneq \frac12(-\phi - iI_\Sigma\phi).
\end{equation*}
Note that there is in fact a map
\begin{equation}
  (\cdot)^*\co \Ad(P^\C) \to \Ad(P^\C)\quad (\xi+i\eta)^* \mapsto (-\xi+i\eta)
\end{equation}
We identify $\varphi$ with the corresponding $G^\C$--equivariant map $P^\C \to \fg^\C$ and we set
\begin{equation*}
  \delbar_I \coloneq \rd + iI\rd.
\end{equation*}
With this notation \autoref{Eq_EBE} can be rewritten as follows.

\begin{prop}
  \label{Prop_SplitEBEIntoHolomorphic+Metric}
  Suppose $(A,\phi,\xi)$ satisfies \autoref{Eq_IDelYPhi=0}.
  The extended Bogomolny equation \autoref{Eq_EBE} holds if and only if
  \begin{gather}
    \label{Eq_EBE_Holomorphic}
    \delbar_I \varphi = 0, \quad
    \sL_{\fd_y}\varphi = 0, \quad
    \sL_{\fd_y}I = 0 \qand \\
    \label{Eq_EBE_Metric}
    i\Lambda(F_A + [\varphi\wedge\varphi^*]) - i\nabla_{A,\del_y} \xi = 0.
  \end{gather}
\end{prop}

\begin{proof}
  Decompose the exterior derivative $\rd_A$ on $\Ad(P)$ as
  \begin{equation*}
    \rd_A = \del_A + \delbar_A + \nabla_{A,\del_y}.
  \end{equation*}  
  By the Kähler identities,
  \begin{equation*}
    \rd_A^*\phi
    = i\Lambda(\delbar_A\varphi + \del_A\varphi^*).
  \end{equation*}
  Since $*_\Sigma = -I$,
  $*_\Sigma\varphi = i\varphi$ and thus
  \begin{equation*}
    *\varphi = i\rd y\wedge \varphi.
  \end{equation*}
  Therefore, the second equation of \autoref{Eq_EBE} is equivalent to
  \begin{align*}
    \delbar_A\varphi - \del_A\varphi^* &= 0, \\
    \nabla_{A,\del_y}\varphi - i[\xi,\varphi] &= 0, \qand\\
    \nabla_{A,\del_y}\varphi^* + i[\xi,\varphi^*] &= 0.
  \end{align*}
  This shows that the last two equations of \autoref{Eq_EBE} are equivalent to the first two equations of \autoref{Eq_EBE_Holomorphic}.

  We have
  \begin{equation}
    *\rd_A\xi = \nabla_{\del_y}\xi\cdot \vol_\Sigma + \rd y \wedge I_\Sigma\rd_A\Sigma.
  \end{equation}
  From this it follows that the part of the first equation \autoref{Eq_EBE} which does not involve the $y$--component is equivalent to \autoref{Eq_EBE_Metric}.
  It remains to identify the part of \autoref{Eq_EBE} which does involve the $y$--component is equivalent the last equation in \autoref{Eq_EBE_Holomorphic}.
  
  Let $v$ be vector field on $\Sigma$.
  Extend it to $[0,1]\times\Sigma$ subject to the condition $[\del_y,v]=0$.
  Denote by $\tilde v$ the horizontal lift of $v$.
  The condition $F_A(\del_y,v) = \rd_A\xi(I_\Sigma v)$ amounts to
  \begin{equation*}
    [\tilde \del_y,\tilde v] = [I \tilde v,\xi].
  \end{equation*}
  Therefore and since $I$ is integrable,
  \begin{align*}
    [\fd_y,I\tilde v]
    &=
      [\tilde\del_y,Iv] - [i\xi,I\tilde v] \\
    &=
      -[\tilde v,\xi] + [I\tilde v,i\xi] \\
    &=
      I([I\tilde v,\xi] + [\tilde v,i\xi]) \\
    &=
      I[\fd_y,\tilde v].
  \end{align*}
  For any $\eta \in \fg^\C$, we have
  \begin{align*}
    [\fd_y,I\eta] = 0 = I [\fd_y,\eta],
  \end{align*}
  because $I\eta=i\eta$ and $\fd_y$ is $G^\C$--equivariant by construction.
  This shows that $\sL_{\fd_y}I = 0$ is equivalent to the part of \autoref{Eq_EBE} which does involve the $y$--component.
\end{proof}


Let $(P,\Psi)$ be a $(p,w)$--framed principal $G$--bundle over $[0,1]\times \Sigma$.
Denote by $P^\C$ the induced principal $G^\C$--bundle.
Denote by $I_w$ and $\delbar_y^w$ the structures induced by the Dirac monopole of coweight $w$.

\begin{definition}
  \label{Def_ParametrizedHeckeModification}
  A \defined{complex triple} on $P^\C$ is a triple $(I,\varphi,\fd_y)$ consisting of:
  \begin{enumerate}
  \item
    an endomorphism $I \in \Gamma(\End(TP^\C))$ which restricts to an complex structure on each $\set{y}\times\Sigma$,
  \item
    a section $\varphi \in \Gamma(\pi_\Sigma^*T^*\Sigma^{1,0}\otimes \Ad(P^\C))$, and
  \item
    a vector field $\fd_y \in \Vect(P^\C)$ which projects to $\del_y$
  \end{enumerate}
  such that there exists $\alpha > 0$ such that
  \begin{equation}
    \label{Eq_ParametrizedHeckeModification_Singularity}
    \Psi_*I = I_w + O(r^\alpha), \quad
    \Psi_*\varphi = O(1), \qandq
    \Psi_*\fd_y = \fd_y^w + O(r^{-1+\alpha}).
  \end{equation}
  Here $r$ is the distance to $p$.

  A complex triple $(\delbar,\varphi,\fd_y)$ satisfying
  \begin{equation}
    \label{Eq_ParametrizedHeckeModification}
    \delbar_I \varphi = 0, \quad
    \sL_{\fd_y}\varphi = 0, \qandq
    \sL_{\fd_y}I = 0
  \end{equation}
  is called a \defined{parametrized Hecke modification}.
\end{definition}

The following observation is fundamental to this article.

\begin{prop}[{\citet[Section 9.1]{Kapustin2007}}]
  \label{Prop_ScatteringMap}
  Let $(I,\varphi,\fd_y)$ be a parametrized Hecke modification.
  Denote by $(\sP_0,\varphi_0)$ and $(\sP_1,\varphi_1)$ the $G^\C$ Higgs bundles induced by restriction to $\set{0}\times\Sigma$ and $\set{1}\times\Sigma$ respectively.
  The diffeomorphism obtained by integrating the vector field $\fd_y$ induces a 
  Hecke modification
  \begin{equation}
    \sigma\co (\sP_0,\varphi_0)|_{\Sigma\setminus\set{z}} \to (\sP_1,\varphi_1)|_{\Sigma\setminus\set{z}}
  \end{equation}
  at $z$ of coweight $w$.
\end{prop}

\begin{definition}
  We call $\sigma$ the \defined{scattering map} associated with $(I,\varphi,\fd_y)$.
\end{definition}

\begin{prop}[{\citet[Section 2.2]{Charbonneau2011}}]
  \label{Prop_DiracMonopoleScatteringMap}
  The scattering map for the Dirac monopole of coweight $w$ on $[-\epsilon,\epsilon]\times\C$ is given by the complexification of $w$ in suitable holomorphic trivializations.
\end{prop}

% XXX: Redo this in the principal bundle setting?

\begin{proof}
  It suffices to consider \autoref{Ex_DiracMonopole}.
  Also, we can work with the complex vector bundle $\pi^*\sO(1)$ associated with $P$.  
  Set
  \begin{equation*}
    U_\pm \coloneq \set{ (y,z) \in \R\times \C : \pm y > 0 }.
  \end{equation*}
  There are trivializations $\tau_\pm\co \pi^*\sO(1)|_{U_\pm} \iso U_\pm\times \C$,
  such that the transition function $\tau \co U_+\cap U_- \to \U(1)$ is given by
  \begin{equation*}
    (y,z) \mapsto (z/\abs{z}).
  \end{equation*}
  That is,    
  \begin{equation*}
    \tau_+\circ \tau_-^{-1}(y,z;w) = (y,z:\tau(y,z)w).
  \end{equation*}
  In these trivializations we have
  \begin{equation*}
    \nabla_{A_\pm} \coloneq (\tau_\pm)_*\nabla_A
    = \rd + \frac{1}{4}(\mp 1 + y/r) \frac{\bar z\rd z - z\rd\bar z}{\abs{z}^2}.
  \end{equation*}

  Since
  \begin{equation*}
    \rd r = \frac{1}{2r}(\bar z \rd z + z\rd\bar z + 2y\rd y),
  \end{equation*}
  the gauge transformation $g_\pm(y,z) = (r\pm y)^{\pm 1/2}$ satisfies
  \begin{align*}
    -(\rd g_\pm)g_\pm^{-1}
    &=
      \pm\frac{1}{2(r \pm y)}(\rd r \pm \rd y) \\
    &=        
      \pm\frac{1}{4r(r\pm y)}(\bar z \rd z + z \rd \bar z + 2(y \pm r)\rd y) \\
    &=
      \frac{1}{4}(\pm 1 + y/r)\frac{\bar z \rd z + z \rd \bar z}{\abs{z}^2} \pm \frac{1}{2r}\rd y.
  \end{align*}    
  Therefore,
  \begin{align*}
    \nabla_{\tilde A_\pm}
    &\coloneq 
      (g_\pm)_*\nabla_{A_\pm} \\
    &=
      \nabla_{A_\pm} - (\rd g_\pm)g_\pm^{-1} \\
    &=
      \rd + \frac{1}{2} (1\pm y/r) \frac{\bar z\rd z}{\abs{z}^2} \pm \frac{1}{2r}\rd y.        
  \end{align*}
  In particular,
  \begin{equation*}
    \delbar_{\tilde A_\pm} = 0 \qandq
    \nabla_{\tilde A_\pm,\del_y} + i\xi = \del_y + (-1\pm 1) \frac{1}{2r}.
  \end{equation*}
  Therefore, the scattering map is given by
  \begin{equation*}
    g_+(-\epsilon,z) \cdot \tau(\epsilon,z) \cdot g_-^{-1}(-\epsilon,z) 
    =
      (r+y)^{1/2}\frac{z}{\abs{z}}(r-y)^{1/2}
    =
    z
  \end{equation*}
  in the holomorphic trivializations.
\end{proof}

\begin{proof}[Proof of \autoref{Prop_ScatteringMap}]
  That $\sigma$ is holomorphic and preserves the Higgs field follows directly from \autoref{Eq_ParametrizedHeckeModification}.
  To prove is given by the complexification of $w$ near $z$ we follow \citet[Proposition 2.5]{Charbonneau2011}.
  It suffices to consider a neighborhood of $p_0$.
  Denote by $(I_w,0,\fd_y^w)$ the model on $P_w^\C$.
  By \autoref{Prop_DiracMonopoleScatteringMap},
  in suitable holomorphic trivializations,
  the scattering map for the model given by the complexification of $w$.

  Choose two sections $s_0$ and $s$ of $P_w^\C$ over $[-\epsilon,0)\times\set{0}$ such that
  \begin{equation*}
    \fd_y^w s_0 = 0, \quad
    \fd_y s = 0, \qandq
    d(s,s_0) = O(r^\alpha).
  \end{equation*}
  Extend $s_0$ and $s$ to sections of $P_w^\C$ over $\sU \coloneq [-\epsilon,\epsilon]\times B_\epsilon(0) \setminus [0,\epsilon]\times\set{0}$ satisfying
  \begin{equation*}
    \fd_y^w s_0 = 0, \quad
    \delbar_{I^w}s_0 = 0, \quad
    \fd_y^w s = 0, \qandq
    \delbar_{I}s = 0.
  \end{equation*}
  These still satisfy
  \begin{equation*}
    d(s,s_0) = O(r^\alpha).
  \end{equation*}

  For each $p = (y,z) \in \sU$,
  there exists a unique $G^\C$--equivariant map $\Phi_p \co P_p^\C \to P_p^\C$ such that
  \begin{equation*}
    s(p) = \Phi(p) \circ s_0(p).
  \end{equation*}
  The induced map $\Phi \co P_p^\C|_{\sU} \to P_p^\C|_{\sU}$ satisfies
  \begin{equation*}
    \Phi_*I_w = I \qandq \Phi_*\fd_y^w = \fd_y.
  \end{equation*}
  Since $d(s,s_0) = O(r^\alpha)$, $\Phi$ extends to all of $[-\epsilon,\epsilon]\times B_\epsilon(0) \setminus \set{(0,0)}$.

  It follows that with respect to the trivializations of $P_w^\C$ in which the model scattering map is given by the $w^\C$ the scattering map for $(I,\phi,\fd_y)$ is given by
  \begin{equation*}
    z \mapsto \Phi(\epsilon,z) w^\C(z) \Phi(-\epsilon,z)^{-1}.
    \qedhere
  \end{equation*}
\end{proof}

The above construction yields a map
\begin{equation}
  S \co \sM^\EBE(A_0,\phi_0;p,w) \to \sM^\Hecke(\sP_0,\varphi_0;z,w)
\end{equation}
defined by
\begin{equation}
  S[A,\phi,\xi] \mapsto [\sigma].
\end{equation}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "HeckeModificationsEBE"
%%% End:
